High-dimensional consistency in score-based and hybrid structure learning

Main approaches for learning Bayesian networks can be classified as constraint-based, score-based or hybrid methods. Although high-dimensional consistency results are available for constraint-based methods like the PC algorithm, such results have not been proved for score-based or hybrid methods, and most of the hybrid methods have not even shown to be consistent in the classical setting where the number of variables remains fixed and the sample size tends to infinity. In this paper, we show that consistency of hybrid methods based on greedy equivalence search (GES) can be achieved in the classical setting with adaptive restrictions on the search space that depend on the current state of the algorithm. Moreover, we prove consistency of GES and adaptively restricted GES (ARGES) in several sparse high-dimensional settings. ARGES scales well to sparse graphs with thousands of variables and our simulation study indicates that both GES and ARGES generally outperform the PC algorithm.

==> texfiles/Consistency.tex <==
\section{Consistency proof}

Let $\mathcal{C}_F$ denote the output of the restricted forward phase. In the restricted forward phase, edges are added one by one as in the forward phase of GES, but at each step an edge between two non-adjacent nodes of the current CPDAG is taken under consideration only if it satisfies one of the following criteria: (i) the nodes are adjacent in the true (or estimated) conditional independence graph (CIG) or (ii) the edge can shield at least one v-structure of the current CPDAG. 

Let $\mathcal{G}$ be the true DAG and $\mathcal{H}$ be a DAG in the Markov equivalence class of $\mathcal{C}_F$. Assume that the scoring criterion is \emph{locally consistent} (see Definition 6 of \cite{Chickering03}). We will show below that in the limit of large sample, $\mathcal{H}$ is an \emph{independence map} of $\mathcal{G}$ (Theorem \ref{theorem: independence map}), i.e., every conditional independence relationship in $\mathcal{H}$ holds in $\mathcal{G}$. Note that the same result has been used in \cite{Chickering03} (while considering $\mathcal{C}_F$ as the output of the forward phase of GES) to prove consistency of GES. Therefore, consistency of our algorithm follows from the proof of Lemma 10 of \cite{Chickering03}, as the backward phase of our algorithm is identical to that of GES.  

We denote the set of parents, descendants and non-descendants of a node $X$ in a DAG $\mathcal{G}$ by $\mathbf{Pa}_{\mathcal{G}}(X)$, $\mathbf{De}_{\mathcal{G}}(X)$ and $\mathbf{Nd}_{\mathcal{G}}(X)$ respectively, where we assume that every node is a descendant of itself. $\pi_{G}(X_1,X_2,\ldots,X_n)$ denotes a path from $X_1$ to $X_n$ in the DAG $\mathcal{G}$. We say that a set $\mathbf{S}$ intersects a path $\pi_{G}(X_1,X_2,\ldots,X_n)$ if $\mathbf{S} \cap \{ X_1,X_2,\ldots,X_n\}$ is non-empty.


We first prove two lemmas which will be used to prove Theorem \ref{theorem: independence map}.

\begin{lemma}\label{lemma: basic properties}
Let $\mathcal{G}$ and $\mathcal{H}$ be as defined above. Then in the limit of large sample the following hold:
\begin{enumerate}
\item $Skeleton(\mathcal{G}) \subseteq Skeleton(\mathcal{H})$;
\item If $W_1 \rightarrow W_2 \leftarrow W_3$ is a v-structure in $\mathcal{G}$, then either $W_1$ and $W_2$ are adjacent in $\mathcal{H}$ or $W_1 \rightarrow W_2 \leftarrow W_3$ is also a v-structure in $\mathcal{H}$.
\end{enumerate}
\end{lemma}
\begin{proof}
Suppose $X$ and $Y$ are adjacent in $\mathcal{G}$ but not in $H$. Without loss of generality, assume that $Y \in \mathbf{Nd}_{\mathcal{H}}(X)$. Then we construct the DAG $\mathcal{H}'$ from $\mathcal{H}$ by adding the edge $Y \rightarrow X$. Now since $Y \nindep X \mid \mathbf{Pa}_{\mathcal{H}}(X)$ and the scoring criterion is locally consistent, in the limit of large sample, $\mathcal{H}'$ has a higher score than $\mathcal{H}$. This contradicts the fact that $\mathcal{C}_{F}$ is the output of the restricted forward phase, since addition of the edge $Y \rightarrow X $ is permissible as $X$ and $Y$ are adjacent in the true DAG and hence in the true CIG. This completes the proof of the first part.

From the first part, it follows that $\pi_{\mathcal{H}}(W_1,W_2,W_2)$ is a path in $\mathcal{H}$. Suppose $W_1$ and $W_2$ are not adjacent in $\mathcal{H}$ and $\pi_{\mathcal{H}}(W_1,W_2,W_2)$ is not a v-structure in $\mathcal{H}$. Without loss of generality, assume that $W_1 \in \mathbf{Nd}_{H}(W_3)$. Thus $\pi_{\mathcal{H}}(W_1,W_2,W_2)$ is either $W_1 \leftarrow W_2 \rightarrow W_3$ or $W_1 \rightarrow W_2 \rightarrow W_3$ and hence $W_2 \in \mathbf{Pa}_{\mathcal{H}}(W_3)$. Therefore, the path $W_1 \rightarrow W_2 \leftarrow W_3$ in $\mathcal{G}$ is not blocked by $\mathbf{Pa}_{\mathcal{H}}(W_3)$ and hence $W_1 \nindep W_3 \mid \mathbf{Pa}_{\mathcal{H}}(W_3)$. Thus, adding the edge $W_1 \rightarrow W_3$ would increase the score in the limit of large sample. This is a contradiction, since $W_1$ and $W_3$ are adjacent in the true CIG (as $W_1 \rightarrow W_2 \leftarrow W_3$ is a v-structure in $\mathcal{G}$).
\end{proof}

\begin{lemma}\label{lemma: v-structure}
Let $\mathcal{H}$ be any DAG and let $\pi_{H}(Z_0,\ldots,Z_{n+1})$ be a path in $\mathcal{H}$. Suppose $Z_0$ and $Z_{n+1}$ are not adjacent in $\mathcal{H}$ and every path $\pi_{H}(Z_0,Z_{r_1},\ldots,Z_{r_m},Z_{n+1})$ where $1\leq r_1 \leq \cdots \leq r_m \leq n+1$, if exists in $\mathcal{H}$, contains a collider. Then there exists $0\leq i < j <k \leq n+1$ such that 
\begin{enumerate}
\item $Z_i \rightarrow Z_j \leftarrow Z_k$ is a v-structure in $\mathcal{H}$, and
\item $Z_{i+1},\ldots,Z_{k-1} \in \mathbf{De}_{\mathcal{H}}(Z_i) \cap \mathbf{De}_{\mathcal{H}}(Z_k)$ and hence $Z_{i+1},\ldots,Z_{k-1} \notin \mathbf{Pa}_{\mathcal{H}}(Z_i) \cup \mathbf{Pa}_{\mathcal{H}}(Z_k)$.
\end{enumerate}
\end{lemma}

\begin{proof}
We prove the result by induction. First note that the case $n=1$ is trivial since $Z_0$ and $Z_{n+1}$ are not adjacent in $\mathcal{H}$. Next, we assume $n>1$ and the result holds for any integer smaller than $n$.

Let $Z_{r-1} \rightarrow Z_{r} \leftarrow Z_{r+1}$ be a collider in $\pi_{\mathcal{H}}(Z_0,\ldots,Z_{n+1})$. Now if $Z_{r-1}$ and $Z_{r+1}$ are not adjacent, we are done. Otherwise, we consider the path $\pi_{\mathcal{H}}(Z_0,\ldots,Z_{r-1},Z_{r+1},\ldots,Z_{n+1})$. Then by the induction hypothesis, there exists a v-structure $Z_i \rightarrow Z_j \leftarrow Z_k$ in $\mathcal{H}$ such that $\{Z_{i+1},\ldots,Z_{k-1}\} \setminus \{ Z_{r}\} \subseteq \mathbf{De}_{\mathcal{H}}(Z_i) \cap \mathbf{De}_{\mathcal{H}}(Z_k)$.

If $i>r$ or $k<r$, we are done. Otherwise, $i+1 \leq r \leq k-1$ and hence $Z_{r-1} \in \mathbf{De}_{\mathcal{H}}(Z_i)$ and $Z_{r+1} \in \mathbf{De}_{\mathcal{H}}(Z_{k})$. Therefore, $Z_r \in \mathbf{De}_{\mathcal{H}}(Z_i) \cap \mathbf{De}_{\mathcal{H}}(Z_k)$, since $Z_{r-1},Z_{r+1} \in \mathbf{Pa}_{\mathcal{H}}(Z_r)$. The last part follows from the fact that $\mathcal{H}$ contains no directed cycle.
\end{proof}

\begin{theorem}\label{theorem: independence map}
Let $\mathcal{G}$ be the true DAG and $\mathcal{H}$ be any DAG in the Markov equivalence class of $\mathcal{C}_{F}$, which is the output of the restricted forward phase. Then in the limit of large sample, $\mathcal{H}$ is an independence map of $\mathcal{G}$.
\end{theorem}

\begin{proof}
Suppose not and thus there exists nodes $X,Y$ and a path $\pi_{G}^{X,Y}$ in $\mathcal{G}$ such that $Y \in \mathbf{Nd}_{\mathcal{H}}(X) \setminus \mathbf{Pa}_{\mathcal{H}}(X)$ and $\pi_{G}^{X,Y}$ is not blocked by $\mathbf{Pa}_{\mathcal{H}}(X)$. Among all such triples $(X,Y,\pi_{\mathcal{G}}^{X,Y})$, we choose one triple $(Z_0,Z_{n+1},\pi_{G}(Z_0,Z_1,\ldots,Z_{n+1}))$ which has the minimum number of colliders. Let $\pi_{G}(Z_0,\ldots,Z_{n+1})$ contain $m$ colliders. Since Lemma \ref{lemma: basic properties} implies $Skeleton(\mathcal{G}) \subseteq Skeleton(\mathcal{H})$, the path $\pi_{\mathcal{H}}(Z_0,\ldots,Z_{n+1})$ exists in $\mathcal{H}$.

We show below that there exists $0\leq i < j <k \leq n+1$ such that $Z_i \rightarrow Z_j \leftarrow Z_k$ is a v-structure in $\mathcal{H}$, and at least one of the following hold:
\begin{description}
\item[(i)] $Z_i \in \mathbf{Nd}_{\mathcal{H}}(Z_k)$ and $\pi_{\mathcal{G}}(Z_i,Z_{i+1},\ldots,Z_k)$ is not blocked by $\mathbf{Pa}_{\mathcal{H}}(Z_k)$ (which implies $Z_i \nindep Z_k \mid \mathbf{Pa}_{\mathcal{H}}(Z_k)$);
\item[(ii)]  $Z_k \in \mathbf{Nd}_{\mathcal{H}}(Z_i)$ and $\pi_{\mathcal{G}}(Z_i,Z_{i+1},\ldots,Z_k)$ is not blocked by $\mathbf{Pa}_{\mathcal{H}}(Z_i)$ (which implies $Z_k \nindep Z_i \mid \mathbf{Pa}_{\mathcal{H}}(Z_i)$).
\end{description}

Note that this is a contradiction since the edge $Z_i \rightarrow Z_k$ (if (i) holds) or $Z_k \rightarrow Z_i$ (if (ii) holds) can be added to shield the v-structure $Z_i \rightarrow Z_j \leftarrow Z_k$ in $\mathcal{H}$ and the resulting DAG would have a higher score than $\mathcal{H}$ in the limit of large sample, since the scoring criterion is locally consistent.

If $m=0$, i.e., $\pi_{G}(Z_0,\ldots,Z_{n+1})$ contains no collider, then $\{Z_1,\ldots,Z_n\} \cap \mathbf{Pa}_{\mathcal{H}}(Z_0) = \emptyset$, since otherwise $\mathbf{Pa}_{\mathcal{H}}(Z_0)$ would block the path $\pi_{G}(Z_0,\ldots,Z_{n+1})$. Hence, every path from $Z_0$ to $Z_{n+1}$ in $\mathcal{H}$ through any subset of $Z_1,\ldots,Z_n$ must contain a collider, since $Z_{n+1} \in \mathbf{Nd}_{\mathcal{H}}(Z_0) \setminus \mathbf{Pa}_{\mathcal{H}}(Z_0)$. Therefore, by Lemma \ref{lemma: v-structure}, there exists a v-structure $Z_{i} \rightarrow Z_{j} \leftarrow Z_k$ ($0\leq i < j <k \leq n+1$) such that $Z_{i+1},\ldots,Z_{k-1} \notin \mathbf{Pa}_{\mathcal{H}}(Z_{i}) \cup \mathbf{Pa}_{\mathcal{H}}(Z_k)$. Then we are done, since without loss of generality we can assume $Z_i \in \mathbf{Nd}_{\mathcal{H}}(Z_k)$ and the path $\pi_\mathcal{G}(Z_i,Z_{i+1},\ldots,Z_k)$ is not blocked by $\mathbf{Pa}_{\mathcal{H}}(Z_k)$.

Therefore, we assume $m\geq 1$ and without loss of generality we further assume that $\{Z_1,\ldots,Z_n\} \setminus \mathbf{Pa}_{\mathcal{H}}(Z_0) \subseteq \mathbf{De}_{\mathcal{H}}(Z_0)$, since otherwise we can consider $Z_{r^*}$ instead of $Z_{n+1}$, where $r^* = \min \{ r \mid Z_{r} \in \mathbf{Nd}_{\mathcal{H}}(Z_0) \setminus \mathbf{Pa}_{\mathcal{H}}(Z_0) \}$.

Now if $Z_r \in \mathbf{Pa}_{\mathcal{H}}(Z_0)$ for some $1\leq r \leq n$, then $Z_r$ must be a collider node in $\pi_{\mathcal{G}}(Z_0,\ldots,Z_{n+1})$, since otherwise $\mathbf{Pa}_{\mathcal{H}}(Z_0)$ would block $\pi_{\mathcal{G}}(Z_0,\ldots,Z_{n+1})$. We show that $Z_{r-1}$ and $Z_{r+1}$ are adjacent in $\mathcal{H}$. If $Z_{r-1}$ and $Z_{r+1}$ are adjacent in $\mathcal{G}$, then so they are in $\mathcal{H}$. Otherwise, $Z_{r-1} \rightarrow Z_r \leftarrow Z_{r+1}$ is a v-structure in $\mathcal{G}$. Moreover, $Z_{r-1}$ is not a collider in $\pi_{\mathcal{G}}(Z_0,\ldots,Z_{n+1})$ and hence $Z_{r-1} \notin \mathbf{Pa}_{\mathcal{H}}(Z_0)$. Thus, by assumption, $Z_{r-1}$ is a descendant of $Z_0$ in $\mathcal{H}$ and hence a descendant of $Z_r$ in $\mathcal{H}$ (as $Z_r \in \mathbf{Pa}_{\mathcal{H}}(Z_0)$). Therefore, the edge between $Z_{r-1}$ and $Z_{r}$ is directed away from $Z_r$ and $\pi_{\mathcal{H}}(Z_{r-1},Z_r,Z_{r+1})$ is not a v-structure. Then the second part of Lemma \ref{lemma: basic properties} implies that $Z_{r-1}$ and $Z_{r+1}$ are adjacent in $\mathcal{H}$.

Therefore, there is a path in $\mathcal{H}$ from $Z_0$ to $Z_{n+1}$ through $\{Z_1,\ldots,Z_{n}\} \setminus \mathbf{Pa}_{\mathcal{H}}(Z_0)$. Since, in $\mathcal{H}$, any path from $Z_0$ to $Z_{n+1}$ that contains no parent of $Z_0$ must contain a collider, Lemma \ref{lemma: v-structure} implies that there exists a v-structure $Z_{i} \rightarrow Z_{j} \leftarrow Z_k$ ($0\leq i < j <k \leq n+1$) in $\mathcal{H}$ such that no parent of $Z_i$ or $Z_k$ belongs to the set $\{Z_{i+1},\ldots,Z_{k-1}\} \setminus \mathbf{Pa}_{\mathcal{H}}(Z_{0})$. Thus no non-collider node in $\pi_{\mathcal{G}}(Z_i,\ldots,Z_k)$ belongs to $\mathbf{Pa}_{\mathcal{H}}(Z_i) \cup \mathbf{\mathcal{H}}(Z_k)$.

If $k=n+1$, $Z_k$ is a non-descendant of $Z_i$, since $Z_{n+1}$ is a non-descendant of $Z_0$ and $Z_i$ is descendant of $Z_0$. Moreover, we will show in Lemma \ref{lemma: descendants of a collider} that if $Z_r$ is a collider in $\pi_{\mathcal{G}}(Z_i,\ldots,Z_{k})$ then $\mathbf{Pa}_{\mathcal{H}}(Z_i) \cap \mathbf{De}_{\mathcal{G}}(Z_r)$ is non-empty. Therefore, the path $\pi_{\mathcal{G}}(Z_i,\ldots,Z_{k})$ is not blocked by $\mathbf{Pa}_{\mathcal{H}}(Z_i)$. Thus, we are done.

Otherwise, if $k\neq n+1$, without loss of generality, we assume $Z_i \in \mathbf{Nd}_{\mathcal{H}}(Z_k)$. Then again Lemma \ref{lemma: descendants of a collider} implies that if $Z_r$ is a collider in $\pi_{\mathcal{G}}(Z_i,\ldots,Z_{k})$ then $\mathbf{Pa}_{\mathcal{H}}(Z_k) \cap \mathbf{De}_{\mathcal{G}}(Z_r)$ is non-empty. Therefore, the path $\pi_{\mathcal{G}}(Z_i,\ldots,Z_{k})$ is not blocked by $\mathbf{Pa}_{\mathcal{H}}(Z_k)$. This completes the proof.
\end{proof}

\begin{lemma}\label{lemma: descendants of a collider}
Let $Z_0$, $Z_{n+1}$ and $\pi_{\mathcal{G}}(Z_0,\ldots,Z_{n+1})$ be as in the proof of Theorem \ref{theorem: independence map} and let $\pi_{\mathcal{G}}(Z_0,\ldots,Z_{n+1})$ contain $m\geq 1$ colliders. Let $Z_i \in \mathbf{De}_{\mathcal{H}}(Z_0)$ and let $Z_r$ be a collider node in $\pi_{\mathcal{G}}(Z_0,\ldots,Z_{n+1})$.  Assume that the sets $\mathbf{Pa}_{\mathcal{H}}(Z_i)$ and $\{Z_{i+1},\ldots,Z_{r}\} \setminus \mathbf{Pa}_{\mathcal{H}}(Z_0)$ (or $\{Z_{r+1},\ldots,Z_{i}\} \setminus \mathbf{Pa}_{\mathcal{H}}(Z_0)$) are disjoint. Then $\mathbf{Pa}_{\mathcal{H}}(Z_i) \cap \mathbf{De}_{\mathcal{G}}(Z_r)$ is non-empty.
\end{lemma}
\begin{proof}
Without loss of generality, we assume $i<r$. Let $\{Z_{\ell_1},\ldots,Z_{\ell_q}\}$ be the set of all collider nodes in $\pi_{\mathcal{G}}(Z_i,\ldots,Z_{r+1})$, where $1 \leq q \leq m$ and $\ell_q = r$. Since the path $\pi_{\mathcal{G}}(Z_0,\ldots,Z_{n+1})$ is not blocked by $\mathbf{Pa}_{\mathcal{H}}(Z_0)$, the following hold:
\begin{description}
\item[(i)]  The set $\{Z_{i+1},\ldots,Z_{r}\} \setminus \{Z_{\ell_1},\ldots,Z_{\ell_q}\}$ does not contain any element of $\mathbf{Pa}_{\mathcal{H}}(Z_0)$ and hence the sets $\mathbf{Pa}_{\mathcal{H}}(Z_i)$ and $\{Z_{i+1},\ldots,Z_{r}\} \setminus \{Z_{\ell_1},\ldots,Z_{\ell_q}\}$ are disjoint (as $\mathbf{Pa}_{\mathcal{H}}(Z_i)$ and $\{Z_{i+1},\ldots,Z_{r}\} \setminus \mathbf{Pa}_{\mathcal{H}}(Z_0)$ are disjoint);
\item[(ii)] For all $j=1,\ldots,q$, the set $\mathbf{Pa}_{\mathcal{H}}(Z_0) \cap  \mathbf{De}_{\mathcal{G}}(Z_{\ell_j})$ is non-empty. Therefore, we can choose $W_j \in \mathbf{Pa}_{\mathcal{H}}(Z_0) \cap  \mathbf{De}_{\mathcal{G}}(Z_{\ell_1})$ and a directed path $\pi_{\mathcal{G}}(Z_{\ell_j},\ldots,W_j)$ from $Z_{\ell_j}$ to $W_j$ in $\mathcal{G}$.
\end{description}

We prove, by induction on $q$, that $\mathbf{Pa}_{\mathcal{H}}(Z_i) \cap \mathbf{De}_{\mathcal{G}}(Z_{\ell_j})$ is non-empty, for all $j=1,\ldots,q$. First, consider the case $q=1$. Let $W_1$ and $\pi_{\mathcal{G}}(Z_{\ell_1},\ldots,W_1)$ be as in (ii). If $\mathbf{Pa}_{\mathcal{H}}(Z_i)$ intersects $\pi_{\mathcal{G}}(Z_{\ell_1},\ldots,W_1)$, we are done. Otherwise, $W_1 \in \mathbf{Nd}_{\mathcal{H}}(Z_i) \setminus \mathbf{Pa}_{\mathcal{H}}(Z_i)$ as $Z_i \in \mathbf{De}_{\mathcal{H}}(Z_0)$. On the other hand, the path $\pi_{\mathcal{G}}(Z_i,\ldots,Z_{\ell_1},\ldots,W_1)$, obtained from concatenating $\pi_{\mathcal{G}}(Z_i,Z_{i+1},\ldots,Z_{\ell_1})$ and $\pi_{\mathcal{G}}(Z_{\ell_1},\ldots,W_1)$, is not blocked by $\mathbf{Pa}_{\mathcal{H}}(Z_i)$ (as it contains no collider and $\mathbf{Pa}_{\mathcal{H}}(Z_i)$ does not intersect the path). This contradicts the special choice of the triple $(Z_0,Z_{n+1},\pi_{\mathcal{G}}(Z_0,\ldots,Z_{n+1}))$, since $\pi_{\mathcal{G}}(Z_i,\ldots,Z_{\ell_1},\ldots,W_1)$ contains no collider and $\pi_{\mathcal{G}}(Z_0,\ldots,Z_{n+1}$ contains $m\geq 1$ colliders.

Next, we assume $q>1$ and $\mathbf{Pa}_{\mathcal{H}}(Z_i) \cap \mathbf{De}_{\mathcal{G}}(Z_{\ell_j})$ is non-empty, for all $j=1,\ldots,q-1$. Let $W_1$ and $\pi_{\mathcal{G}}(Z_{\ell_1},\ldots,W_1)$ be as in (ii). If $\mathbf{Pa}_{\mathcal{H}}(Z_i)$ intersects $\pi_{\mathcal{G}}(Z_{\ell_q},\ldots,W_q)$, we are done. Otherwise, $W_q \in \mathbf{Nd}_{\mathcal{H}}(Z_i) \setminus \mathbf{Pa}_{\mathcal{H}}(Z_i)$. Note that the path $\pi_{\mathcal{G}}(Z_i,\ldots,Z_{\ell_q},\ldots,W_q)$ contains $q-1<m$ colliders nodes, namely $Z_{\ell_1},\ldots,Z_{\ell_{q-1}}$. Thus we complete the proof by showing that $\pi_{\mathcal{G}}(Z_i,\ldots,Z_{\ell_q},\ldots,W_q)$ is not blocked by $\mathbf{Pa}_{\mathcal{H}}(Z_i)$, as this contradicts the special choice of the triple $(Z_0,Z_{n+1},\pi_{\mathcal{G}}(Z_0,\ldots,Z_{n+1}))$. 

The induction hypothesis implies that $\mathbf{Pa}_{\mathcal{H}}(Z_i)$ intersects the set of descendants of every collider node in $\pi_{\mathcal{G}}(Z_i,\ldots,Z_{\ell_q},\ldots,W_q)$. On the other hand, $\mathbf{Pa}_{\mathcal{H}}(Z_i)$ does not intersect the sub-path $\pi_{\mathcal{G}}(Z_{\ell_q},\ldots,W_q)$ (by our assumption) and (i) implies no non-collider node in the sub-path $\pi_{\mathcal{G}}(Z_i,\ldots,Z_{\ell_q -1})$ belongs to $\mathbf{Pa}_{\mathcal{H}}(Z_i)$. Therefore, $\mathbf{Pa}_{\mathcal{H}}(Z_i)$ does not block the path $\pi_{\mathcal{G}}(Z_i,\ldots,Z_{\ell_q},\ldots,W_q)$.

\end{proof}









==> texfiles/high-dim_consistency_old.tex <==
\section{High-dimensional consistency \textcolor{red}{of GES and ARGES} in the multivariate Gaussian setting}\label{section: high-dimensional consistency}
We now consider an asymptotic scenario where the number of variables in $\mathbf{X}$ and the distribution of $\mathbf{X}$ are allowed to change with $n$. Thus, let $\{\mathbf{X}_n \}$ be a sequence of random vectors such that the distribution of each $\mathbf{X}_n$ is \textcolor{red}{multivariate Gaussian and DAG-perfect}. Further, we slightly modify Notation \ref{notation: true graphs} as follows.

\begin{notation}\label{notation: high-dim} We reserve the notation $F_n$, $\mathcal{G}_{n0}$, $\mathcal{C}_{n0}$, $\mathcal{I}_{n0}$ and $\mathcal{D}_n$ for the following: $F_n$ denotes the distribution of $\mathbf{X}_n = (X_{n1},\ldots,X_{np_n })^T$, $\mathcal{G}_{n0}$ denotes a perfect map of $F_n$,  $\mathcal{C}_{n0} = \CPDAG(\mathcal{G}_{n0})$ is the corresponding CPDAG,
  $\mathcal{I}_{n0}$ is the CIG of $F_n$,
  and $\mathcal D_n$ denotes the data, consisting of $n$ i.i.d.\ observations from $F_n$.
\end{notation}

%We show high-dimensional consistency of GES and ARGES under an $\ell_0$-penalized log-likelihood scoring criterion, which is given by Definition \ref{definition: penalized likelihood score}. In Section \ref{subsection: high-dimensional consistency of ARGES}, we prove high-dimensional consistency of ARGES (see Theorem \ref{theorem: high-dimensional consistency of ARGES}). In the following subsection, we state the high-dimensional consistency results of GES and point out required modification of assumptions to follow the same arguments given in the proof of Theorem \ref{theorem: high-dimensional consistency of ARGES}.

We prove high-dimensional consistency of (AR)GES with an $\ell_0$-penalized log-likelihood scoring criterion $\mathcal{S}_{\lambda_n}$ (Definition \ref{definition: penalized likelihood score}), using the following steps. We define a collection of oracle versions of (AR)GES, and prove soundness of them for all $n$, under the oracle scoring criterion $\mathcal{S}_{\lambda_n}^*$ (Definition \ref{definition: oracle score}) for a suitably chosen sequence of penalty parameters $\lambda_n$. We complete the proof by showing that the sample version of (AR)GES with scoring criterion $\mathcal{S}_{\lambda_n}$ is identical to one of the oracle versions (Definition \ref{definition: oracle versions of ARGES}) with probability approaching one, for a suitably chosen sequence of penalty parameters $\lambda_n$.

%in Section \ref{A2-subsection: high-dimensional consistency proof} of \cite{NandyHauserMaathuis15b}
\subsection{$\ell_0$-penalized log-likelihood score in the multivariate Gaussian setting}\label{subsection: l0 penalized likelihood score}

\begin{definition}\label{definition: penalized likelihood score}
Let $\mathcal{H}_n = (\mathbf{X}_n,E_n)$ be a DAG with vertex set $\mathbf{X}_n$ and edge set $E_n$. The $\ell_0$-penalized log-likelihood score with penalty parameter $\lambda_n$ is given by
\begin{align*}%\label{eq: l0-penalized log likelihood}
\mathcal{S}_{\lambda_n}(\mathcal{H}_n,\mathcal{D}_n) = -  \sum_{i=1}^{p_n}\frac{1}{n} \log \left(L(\hat{\boldsymbol\theta}_{ni}(\mathcal{H}_n),\mathcal{D}_n(X_{ni})|\mathcal{D}_n(\mathbf{Pa}_{\mathcal{H}_n}(X_{ni})))\right) + \lambda_n |E_n|,
\end{align*}
where $L({\boldsymbol\theta}_{ni}(\mathcal{H}_n),\mathcal{D}_n(X_{ni})|\mathcal{D}_n(\mathbf{Pa}_{\mathcal{H}_n}(X_{ni})))$ is the likelihood function that corresponds to the conditional density of $X_{ni}$ given $\mathbf{Pa}_{\mathcal{H}_n}(X_{ni})$ and $$\hat{\boldsymbol\theta}_{ni}(\mathcal{H}_n) = \mathop{\mathrm{argmax}}_{{\boldsymbol\theta}_{ni}(\mathcal{H}_n)}~ \frac{1}{n} \log \Big(L({\boldsymbol\theta}_{ni}(\mathcal{H}_n),\mathcal{D}_n(X_{ni})|\mathcal{D}_n(\mathbf{Pa}_{\mathcal{H}_n}(X_{ni}))) \Big)$$ is the maximum likelihood estimate (MLE) of the parameter vector $\boldsymbol\theta_{ni}(\mathcal{H}_n)$.
\end{definition}

\begin{remark}\label{remark: BIC}
The BIC criterion is a special case of the $\ell_0$-penalized log-likelihood score. In particular, the BIC score of a DAG $\mathcal{H}_n$ equals $2n\mathcal{S}_{\lambda_n}(\mathcal{H}_n,\mathcal{D}_n)$ with $\lambda_n = \frac{\log(n)}{2n}$.
\end{remark}

The following lemma shows that when the distribution of $\mathbf{X}_n$ is multivariate Gaussian and $\lambda_n$ is suitably chosen, the $\ell_0$-penalized log-likelihood score of a DAG $\mathcal{H}_n$ can be improved by adding an edge $X_{ni} \rightarrow X_{nj}$ if and only if the sample partial correlation between $X_{ni}$ and $X_{nj}$ given $ \mathbf{Pa}_{\mathcal{H}_n}(X_{nj})$ is nonzero. This is one of the key results for our proof of high-dimensional consistency of (AR)GES.


%the score difference between two DAGs $\mathcal{H}_n$ and $\mathcal{H}_n'$ such that $\mathcal{H}_n'$ is same as $\mathcal{H}_n$ but contains exactly one additional edge, can be written as a function of sample partial correlation.
\begin{lemma}\label{lemma: score difference}
Let $\mathcal{H}_n = (\mathbf{X}_n,E_n)$ be a DAG such that $X_{ni}\in \mathbf{Nd}_{\mathcal{H}_n}(X_{nk})\setminus \mathbf{Pa}_{\mathcal{H}_n}(X_{nk})$. Let $\mathcal{H}_n'=(\mathbf{X}_n,E_n\cup \{X_{ni} \rightarrow X_{nk}\})$. If the distribution of $\mathbf{X}_n$ is multivariate Gaussian, then the $\ell_0$-penalized log-likelihood score difference between $\mathcal{H}_n'$ and $\mathcal{H}_n$ is
\begin{align}\label{eq: score difference formula}
\mathcal{S}_{\lambda_n}(\mathcal{H}_n',\mathcal{D}_n) - \mathcal{S}_{\lambda_n}(\mathcal{H}_n,\mathcal{D}_n) = \frac{1}{2}\log \left(1 - \hat{\rho}_{nik|\mathbf{Pa}_{\mathcal{H}_n}(k)}^2\right) + \lambda_n,
\end{align}
where $\hat{\rho}_{nik|\mathbf{Pa}_{\mathcal{H}_n}(k)}$ denotes the sample partial correlation between $X_{ni}$ and $X_{nk}$ given $ \mathbf{Pa}_{\mathcal{H}_n}(X_{nk})$.
%where $\rho_{nij | S}$ denotes the sample partial correlation between $X_{ni}$ and $X_{nj}$ given $\{X_{nr} : r \in S\}$ and $\mathbf{Pa}_{\mathcal{H}_n(i)} = \{ r : X_{nr} \in \mathbf{Pa}_{\mathcal{H}_n}(X_{ni}) \}$.
\end{lemma}

The first term on the right-hand side of \eqref{eq: score difference formula} equals the negative of the conditional mutual information between $X_{ni}$ and $X_{nk}$ given $\mathbf{Pa}_{\mathcal{H}_n}(X_{nk})$. Thus, Lemma \ref{lemma: score difference} shows that score-based methods like GES essentially use conditional independence tests (cf.\ \cite{AnandkumarEtAl12}) for sequentially adding and deleting edges starting from an initial graph. This shows that the score-based GES algorithm and the constraint-based PC algorithm use the same basic principle (a conditional independence test) in the multivariate Gaussian setting. Although this connection (see Section \ref{section: discussion} for more details) between PC and GES is not very surprising, we were unable to find it in the literature.

Further, Lemma \ref{lemma: score difference} also opens the possibility to define generalized scoring criterions, by replacing the Gaussian conditional mutual information in (2) with a more general measure of conditional independence. In fact, we exploit this in Section 6 to extend our high-dimensional consistency results to nonparanormal distributions.

%\begin{remark}\label{remark: connection between GES and PC}
%Lemma \ref{lemma: score difference} shows that the score-based GES algorithm and the constraint-based PC algorithm are in fact closely related approaches in the multivariate Gaussian setting. The fundamental principle of the PC algorithm is to start with a complete graph and to delete edges sequentially by testing conditional independencies. In the multivariate Gaussian setting, conditional independence tests are equivalent to tests for zero partial correlations. Lemma \ref{lemma: score difference} shows that GES also checks if sample partial correlations are large enough in order to add edges in the forward phase or small enough to delete edges in the backward phase. Although this connection between PC and GES is not very surprising, we were unable to find it in the literature. This also opens the possibility to define generalized scoring criterions by replacing partial correlations with other measures of conditional independence. We exploit this in Section \ref{section: high dimensional consistency in the NPN setting} to extend our high-dimensional consistency results to nonparanormal distributions.
%\end{remark}

We define an oracle version of the $\ell_0$- penalized log-likelihood scoring criterion by replacing the log-likelihood in Definition \ref{definition: penalized likelihood score} by its expectation with respect to the distribution $F_n$ of $\mathbf{X}_n$. The oracle score given by Definition \ref{definition: oracle score} will be used to define a collection of oracle versions of (AR)GES in Section \ref{subsection: high-dimensional consistency of ARGES}.

\begin{definition}\label{definition: oracle score} (Oracle score)
Let $\mathcal{H}_n = (\mathbf{X}_n,E_n)$ be a DAG with vertex set $\mathbf{X}_n$ and edge set $E_n$. We define the oracle score of $\mathcal{H}_n$ with respect to the distribution $F_n$ of $\mathbf{X}_n$ as
\begin{align*}%\label{eq: l0-penalized log likelihood}
\mathcal{S}_{\lambda_n}^*(\mathcal{H}_n,F_n) = -  \sum_{i=1}^{p_n} \Exp \left[ \log \left(L({\boldsymbol\theta}_{ni}^*(\mathcal{H}_n),X_{ni}|\mathbf{Pa}_{\mathcal{H}_n}(X_{ni}))\right) \right] + \lambda_n |E_n|,
\end{align*}
where $L({\boldsymbol\theta}_{ni},X_{ni}|\mathbf{Pa}_{\mathcal{H}_n}(X_{ni}))$ is the likelihood function that corresponds to the conditional density of $X_{ni}$ given $\mathbf{Pa}_{\mathcal{H}_n}(X_{ni})$ and $${\boldsymbol\theta}_{ni}^*(\mathcal{H}_n) = \underset{{\boldsymbol\theta}_{ni}}{\mathrm{argmax}}~  \Exp \left[ \log \left( L({\boldsymbol\theta}_{ni},X_{ni}|\mathbf{Pa}_{\mathcal{H}_n}(X_{ni}))\right) \right].$$
\end{definition}

%\begin{remark}\label{remark: score equivalence}
%Note that both $\mathcal{S}_{\lambda_n}$ (given by Definition \ref{definition: penalized likelihood score}) and $\mathcal{S}_{\lambda_n}^*$ (given by Definition \ref{definition: oracle score}) are decomposable. Moreover, they are score equivalent when the distribution $F_n$ is multivariate Gaussian.
%\end{remark}

We note that both $\mathcal{S}_{\lambda_n}$ and $\mathcal{S}_{\lambda_n}^*$ are decomposable \textcolor{red}{(see Definition \ref{A2-definition: decomposable} of the supplementary material)}. Moreover, they are score equivalent \textcolor{red}{(see Definition \ref{A2-definition: score equivalent} of the supplementary material)} when the distribution $F_n$ is multivariate Gaussian. The scoring criterion used to compute the large sample outputs in Example \ref{example: inconsistency} equals $\mathcal{S}_{\lambda_n}^*$ with $\lambda_n = 0$ (see Section \ref{A2-subsection: limit computation} of the supplementary material).

The following lemma is analogous to Lemma \ref{lemma: score difference}. We do not provide a proof of Lemma \ref{lemma: oracle score difference}, since it can be obtained from the proof of Lemma \ref{lemma: score difference} by replacing the sample quantities by the corresponding population quantities (e.g.\ averages should be replaced by expectations and sample regression coefficients should be replaced by their population counterparts).

\begin{lemma}\label{lemma: oracle score difference}
Let $\mathcal{H}_n = (\mathbf{X}_n,E_n)$ be a DAG such that $X_{ni} \in \mathbf{Nd}_{\mathcal{H}_n}(X_{nk})\setminus \mathbf{Pa}_{\mathcal{H}_n}(X_{nk})$. Let $\mathcal{H}_n'=(\mathbf{X}_n,E_n\cup \{X_{ni} \rightarrow X_{nk}\})$. If the distribution $\mathbf{X}_n$ is multivariate Gaussian, then the oracle score difference between $\mathcal{H}_n'$ and $\mathcal{H}_n$ is
\begin{align*}
\mathcal{S}_{\lambda_n}^*(\mathcal{H}_n',F_n) - \mathcal{S}_{\lambda_n}^*(\mathcal{H}_n,F_n) = \frac{1}{2}\log \left(1 - \rho_{nik|\mathbf{Pa}_{\mathcal{H}_n}(k)}^2\right) + \lambda_n,
\end{align*}
where $\rho_{nik|\mathbf{Pa}_{\mathcal{H}_n}(k)}$ denotes the partial correlation between $X_{ni}$ and $X_{nk}$ given $ \mathbf{Pa}_{\mathcal{H}_n}(X_{nk})$.
%where $\rho_{nij | S}$ denotes the sample partial correlation between $X_{ni}$ and $X_{nj}$ given $\{X_{nr} : r \in S\}$ and $\mathbf{Pa}_{\mathcal{H}_n(i)} = \{ r : X_{nr} \in \mathbf{Pa}_{\mathcal{H}_n}(X_{ni}) \}$.
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{High-dimensional consistency of (AR)GES}\label{subsection: high-dimensional consistency of ARGES}
%Recall that GES can be viewed as a special case of ARGES based on the complete undirected graph ( see end of Section ...).
%Since we do not require any sparsity assumption on the estimated CIG or the estimated CPDAG-skeleton for high-dimensional consistency of ARGES (Theorems \ref{theorem: high-dimensional consistency of ARGES} and \ref{theorem: high-dimensional consistency of ARGES-skeleton}), high-dimensional consistency of GES (Theorem \ref{theorem: high-dimensional consistency of GES}) follows from Theorem \ref{theorem: high-dimensional consistency of ARGES} (or Theorem \ref{theorem: high-dimensional consistency of ARGES-skeleton}).

% Theorem \ref{theorem: high-dimensional consistency of ARGES} or from Theorem \ref{theorem: high-dimensional consistency of ARGES-skeleton}.

First, we define a collection of oracle versions of (AR)GES using the oracle scoring criterion $\mathcal{S}_{\lambda_n}^*$ (Definition \ref{definition: oracle score}). Every move in the forward or backward phase of (AR)GES from a CPDAG $\mathcal{C}_\text{current}$ to $\mathcal{C}_\text{new}$ corresponds to an edge addition or edge deletion in a DAG in the Markov equivalence class of $\mathcal{C}_{\text{current}}$, and thus corresponds to a partial correlation, by Lemma \ref{lemma: oracle score difference}. We denote the partial correlation associated with a move from $\mathcal{C}_\text{current}$ to $\mathcal{C}_\text{new}$ by $\rho(\mathcal{C}_\text{current},\mathcal{C}_\text{new})$.

%We note that the backward phase of (AR)GES with the scoring criterion $\mathcal{S}_{\lambda_n}^*$ is generally not unique, since there can be more than one choice of $\mathcal{C}_\text{new}$ at every step such that $\rho(\mathcal{C}_\text{current},\mathcal{C}_\text{new}) = 0$ for each of them. Further, 

At every step in the forward phase of (AR)GES, an optimal CPDAG is chosen among a set of possible choices for the next step (see line \ref{line: optimal choice 1} of Algorithm \ref{algorithm: the forward phase of ARGES}). These optimal choices in the forward phase are not crucial for consistency of (AR)GES \textcolor{red}{\citep{ChickeringMeek02}}. Thus, we define below oracle versions of (AR)GES that allow sub-optimal choices for edge additions. One of our assumptions (see (A5) below) will be based on this definition.

\begin{definition}\label{definition: oracle versions of ARGES} ($\delta$-optimal oracle versions of (AR)GES)
Let $\delta \in [0,1]$. A $\delta$-optimal oracle version of (AR)GES with scoring criterion $\mathcal S^*_{\lambda}$ consists of two phases: a $\delta$-optimal oracle forward phase and an oracle backward phase. A $\delta$-optimal oracle forward phase of (AR)GES is Algorithm \ref{algorithm: the forward phase of ARGES} based on $\mathcal{I}_{n0}$ (for ARGES-CIG) or $\skeleton(\mathcal{C}_{n0})$ (for ARGES-skeleton) or the complete undirected graph (for GES) using the oracle scoring criterion $\mathcal{S}_{\lambda_n}^*$ depending on $F_n$, where at each step with $\mathfrak{C} \neq \emptyset$ (see line \ref{line: optimal choice 1} of Algorithm \ref{algorithm: the forward phase of ARGES}) $\mathcal{C}_\text{new}$ is chosen to be any CPDAG in $\mathfrak{C}$ such that
\vspace{-0.1in}
$$ |\rho(\mathcal{C}_\text{current},\mathcal{C}_\text{new}) |  \geq \underset{\mathcal{C} \in \mathfrak{C}}{\max} |\rho(\mathcal{C}_\text{current},\mathcal{C}) | - \delta_n. \vspace{-0.05in}$$
%MM: why absolute values on the left side?
An oracle backward phase of (AR)GES equals the backward phase of GES (Algorithm \ref{A2-algorithm: backward phase of GES}), 
% is the same as the backward phase of (AR)GES 
with the oracle scoring criterion $\mathcal{S}_{\lambda_n}^*$. If there are several CPDAGs with the same optimal score, then one of these is chosen arbitrarily as $\mathcal{C}_\text{new}$. 

%, where at every step an arbitrary choice is made to move from $\mathcal{C}_\text{current}$ to $\mathcal{C}_\text{new}$ whenever an optimal move is not uniquely defined. % there are more than one CPDAG $\mathcal{C}$ for which $\rho(\mathcal{C}_\text{current},\mathcal{C}) = 0$.

%A $\delta_n$-optimal oracle version of ARGES based on the complete undirected graph is a $\delta_n$-optimal oracle version of GES.
%A two-phase procedure comprising such a variant of Algorithm \ref{algorithm: the forward phase of ARGES}, and a variant of Algorithm \ref{A2-algorithm: the backward phase of ARGES} of \cite{NandyHauserMaathuis15b} where any edge deletion that decreases the score is allowed, is an oracle version of ARGES if the scoring criterion is given by Definition \ref{definition: oracle score} and a super-graph of $\mathcal{I}_{n0}$ given as an input of Algorithm \ref{algorithm: the forward phase of ARGES}.
%For $\delta = 0$, a $\delta$-optimal oracle version of ARGES is identical to ARGES with an oracle scoring criterion $\mathcal{S}_{\lambda_n}^*$ and we will refer to it as a non-optimal oracle version.
\end{definition}

{\color{red}
\begin{theorem}\label{theorem: soundness of oracle versions} (Soundness)
Fix $n \in \mathbb{N}$ and $\delta_n \in [0,1]$. Let $m_n$ be such that the maximum degree in the output of the forward phase of every $\delta_n$-optimal oracle version of (AR)GES with scoring criterion $\mathcal{S}_{\lambda_n}^*$  is bounded by $m_n$ for all $\lambda_n \geq 0$. If $\lambda_n < - \frac{1}{2}\log(1 - \rho_{nij|S}^2)$ for all $i,j \in \{1,\ldots, p_n\}$ and $S \subseteq  \{1,\ldots, p_n\}\setminus\{i,j\}$ such that $|S| \leq m_n$ and $\rho_{nij|S} \neq 0$, then the outputs of all $\delta_n$-optimal oracle versions of (AR)GES with scoring criterion $\mathcal{S}_{\lambda_n}^*$ are identical and equal to $\mathcal{C}_{n0}$.
\end{theorem}
}

Note that the edge additions in the forward phase of a $\delta_n$-optimal oracle version of (AR)GES are only slightly sub-optimal for small values of $\delta_n$. In fact, we let $\delta_n$ tend to zero as $n \rightarrow \infty$ in assumption (A5) below.  For $\delta_n = 0$, we refer to the forward phase of the $\delta_n$-optimal oracle version of (AR)GES as the oracle forward phase of (AR)GES.\\


%the forward phase of $\delta$-optimal oracle version of (AR)GES is identical to (AR)GES with the oracle scoring criterion $\mathcal{S}_{\lambda_n}^*$ and we will refer to it as the oracle version.


We make the following assumptions to prove high-dimensional consistency of (AR)GES. % under a $\ell_0$-penalized log-likelihood scoring criterion (see Section \ref{subsection: l0 penalized likelihood score}).

\begin{description}
   \item[(A1)] (Gaussianity) The distribution of $\mathbf{X}_n$ is multivariate Gaussian \textcolor{red}{and DAG-perfect} for all $n$;
   \item[(A2)] (high-dimensional setting) $p_n = \mathcal{O}(n^{a})$ for some $0 \leq a < \infty$;
   \item[(A3)]\label{assumption 3} (sparsity condition) Let $q_n = \max_{1 \leq i \leq p_n} |\mathbf{Adj}_{\mathcal{C}_{n0}}(X_{ni})|$ be the maximum degree in $\mathcal{C}_{n0}$.  Then $q_n = \mathcal{O}(n^{1-b_1})$ for some $0 < b_1 \leq 1$;
  % , where $\mathbf{Adj}_{\mathcal{I}_{n0}}(X_i)$ denotes the adjacency set of node $X_{ni}$ in $\mathcal{I}_{n0}$
     \item[(A4)] (consistent estimators of the CIG or the CPDAG-skeleton) There exists a sequence of estimators $\hat{\mathcal{I}}_n$ (for ARGES-CIG) or a sequence of estimators $\hat{\mathcal{U}}_n$ (for ARGES-skeleton) such that \vspace{-0.05in}$$\textcolor{red}{\underset{n \to \infty}{\lim}~\Prob (\hat{\mathcal{I}}_n = \mathcal{I}_{n0}) = 1~\text{or}~ \underset{n \to \infty}{\lim}~\Prob (\hat{\mathcal{U}}_n = \skeleton(\mathcal{C}_{n0})) = 1};$$ %$\Prob ( \max_{1 \leq i \leq p_n} |\mathbf{Adj}_{\hat{\mathcal{I}}_{n}}(X_{ni})| \leq K_1q_n) \rightarrow 1$ for some $K_1\geq1$, and
%      \item[(A5)] (bound on the adaptive part of ARGES) Let $\hat{\mathcal{C}}_n^f(\lambda)$ denote the output of the forward phase of ARGES with the scoring criterion $\mathcal{S}_{\lambda}$ and let $\hat{q}^*_n(\lambda) = \max_{1 \leq i \leq p_n} |\mathbf{Adj}_{\hat{\mathcal{C}}_n^f(\lambda)}(X_{ni})|$.
%      %Further, let $\tilde{\mathcal{C}}_n^{f}(\lambda)$ denote the output of the forward phase of RGES, where RGES is same as ARGES but without the adaptive part and let $\tilde{q}^*_n(\lambda) = \max_{1 \leq i \leq p_n} |\mathbf{Adj}_{\tilde{\mathcal{C}}_n^f(\lambda)}(X_{ni})|$.
%      Then for any sequence $\{\lambda_n\}$ such that $n^{\min(a,b)} \lambda_n \rightarrow \infty$ where $0 < a,b \leq 1$ are as in (A2) and (A3), $\mathbb{P}(\hat{q}^*_n(\lambda_n) \leq K_2  \max_{1 \leq i \leq p_n} |\mathbf{Adj}_{\hat{\mathcal{I}}_{n}}(X_{ni})|) \rightarrow 1$ for some $K_2>0$.

%	\item[(A5)] (bounds on the growth of oracle versions) The maximum degree in the output of the forward phase of every $\delta_n$-optimal oracle version of (AR)GES based on $\hat{\mathcal{I}}_n$ (for ARGES-CIG), based on $\hat{\mathcal{U}}_n$ (for ARGES-skeleton), or based on the complete undirected graph (for GES) is bounded by $K_nq_n$, for some sequences $\delta_n^{-1} = \mathcal{O}(n^{d_1})$ and $K_n =  \mathcal{O}(n^{b_1-b_2})$ such that $0 \leq d_1 < b_2/2$ and $0<b_2 \leq b_1$, where $q_n$ and $ b_1$ are given by (A3).
	
	\item[(A5)] (bounds on the growth of oracle versions) \textcolor{red}{The maximum degree in the output of the forward phase of every $\delta_n$-optimal oracle version of (AR)GES is bounded by $K_nq_n$, for some sequences $\delta_n \rightarrow 0$ and $\{K_n\}$ such that $\delta_n^{-1} = \mathcal{O}(n^{d_1})$ and $K_n =  \mathcal{O}(n^{b_1-b_2})$ for some constants $b_2$ and $d_1$ satisfying $0 \leq d_1 < b_2/2 \leq b_1/2$, where $q_n$ and $ b_1$ are given by (A3).}
%such that $0 \leq d_1 < b_2/2$ and $0<b_2 \leq b_1$
	
   \item[(A6)] (bounds on partial correlations) The partial correlations $\rho_{nij | S}$ between $X_{ni}$ and $X_{nj}$ given $\{X_{nr} : r \in S\}$ satisfy the following upper and lower bounds for all $n$, uniformly over $i,j \in \{1,\ldots,p_n \}$ and $S \subseteq \{1,\ldots,p_n\}\setminus \{ i,j\}$ such that $|S|\leq K_nq_n$ (where $K_n$ and $q_n$ are from (A3) and (A5)):\vspace{-0.05in}
   \begin{align*}
    \mathop{\sup}_{i\neq j, S} |\rho_{nij | S}| \leq M < 1,  ~~ \text{and} ~~  \mathop{\inf}_{i, j, S} \{|\rho_{nij | S}| : \rho_{nij | S} \neq 0 \} \geq c_n,\vspace{-0.05in}
   \end{align*}
   for some sequence \textcolor{red}{$c_n \to 0$} such that $c_n^{-1} = \mathcal{O}(n^{d_2})$ for some constant $d_2$ satisfying $0 <d_2< b_2/2$, where $b_2$ is given by (A5).
%
%      \item[(A6)] \textcolor{red}{(a weaker alternative)} $$\mathbf{S}_r^{\delta_n} := \{\mathbf{Adj}_{\mathcal{C}_{n}^f}(X_{nr}) : \text{$\mathcal{C}_{n}^f $ is an output of an $\delta_n$-optimal oracle versions of ARGES} \}.$$The partial correlations $\rho_{nij | S}$ between $X_{ni}$ and $X_{nj}$ given $\{X_{nr} : r \in S\}$ satisfy the following upper and lower bounds for all $n$:\vspace{-0.05in}
%   \begin{align*}
% &\sup\{|\rho_{nij | S}| : S \subseteq S_j^{\delta_n}, S_j^{\delta_n} \in \mathbf{S}_j^{\delta_n}, i \neq j\} \leq M < 1,  ~~ \text{and}\\
% &\inf\{|\rho_{nij | S}| : S \subseteq S_j^{\delta_n}, S_j^{\delta_n} \in \mathbf{S}_j^{\delta_n}, i \neq j, \rho_{nij | S} \neq 0 \} \geq c_n,\vspace{-0.05in}
%   \end{align*}
%   with $c_n^{-1} = \mathcal{O}(n^{d_2})$ for some $0 \leq d_2 < b_2/2$ where $0 < b_2\leq b_1 \leq 1$ are as in (A5) and (A3).
\end{description}

\cite{KalischBuehlmann07a} proved high dimensional consistency of the PC algorithm assuming (A1), (A2), (A3) and a slightly weaker version of (A6). More precisely, the authors assumed (A6) with $d_2 <b_1/2$. The most criticized assumption among these four assumptions is probably (A6) \citep{UhlerEtAl13}, which is also known as the restricted strong faithfulness condition. Interestingly, \cite{VandeGeerBuhlmann13} proved high-dimensional consistency of the global optimum of the $\ell_0$-penalized likelihood score function without assuming restricted strong faithfulness, but assuming a permutation beta-min condition. Unfortunately, we cannot guarantee that a greedy search method like (AR)GES can always find the global optimum without (A6) and thus we cannot substitute the restricted strong faithfulness assumption here. %We remark that although $\mathcal{O}(p_n^{K_nq_n+2})$ partial correlations appear in (A6), any run of (AR)GES only uses $\mathcal{O}(p_n^22^{K_nq_n})$ of them (see the proof of Theorem \ref{theorem: high-dimensional consistency of ARGES}).

We make two additional assumptions compared to \cite{KalischBuehlmann07a}, namely (A4) and (A5). Assumption (A4) is natural and
%it was also assumed to prove consistency of ARGES in the classical setting (see Theorems \ref{theorem: consistency of ARGES} and \ref{theorem: consistency of ARGES-skeleton}). % since we mainly restrict our search space to an estimated CIG or to an estimated CPDAG-skeleton.
it is not a strong assumption, since there are various estimation methods for the CIG or the CPDAG-skeleton that are consistent in sparse high-dimensional settings (e.g., \cite{MeinshausenBuehlmann06, BanerjeeEtAl08, FriedmanEtAl08, RavikumarEtAl08, RavikumarEtAl11, CaiEtAl12, KalischBuehlmann07a, HaEtAl15}). \textcolor{red}{We require (A5) to avoid estimating those partial correlations that include conditioning sets larger than the sample size $n$. We will discuss (A5) further in Section \ref{subsection: assumption A5} below.}



%, and that (A5) holds for one of the three algorithms does not necessarily imply that it holds for the others.}

%Finally, note that the restricted versions of GES (i.e., ARGES without the adaptive part) satisfy (A4), if $\max_{1 \leq i \leq p_n} |\mathbf{Adj}_{\hat{\mathcal{I}}_n}(X_{ni})| \leq K_n q_n$ (which is a reasonable assumption when $\mathcal{I}_{n0}$ is sufficiently sparse and $\hat{\mathcal{I}}_n$ is a consistent estimator) or if $\max_{1 \leq i \leq p_n} |\mathbf{Adj}_{\hat{\mathcal{U}}_n}(X_{ni})| \leq K_n q_n$ (which is a reasonable assumption because we assume (A2) and $\hat{\mathcal{U}}_n$ can be chosen to be a consistent estimator).

 %Also, note that (A3) is implicitly contained in (A4).
% While it is hard to characterize under which conditions (A5) holds, this assumption can be verified to some extent, by comparing the estimated CIG and the skeleton of the output of the forward phase of ARGES.
%We believe that (A5) generally holds in sparse settings, and the same is indicated by our comparison of ARGES and RGES in simulations.

%Our main theorem is the following and we prove Theorem \ref{theorem: high-dimensional consistency of ARGES} in Section \ref{A2-subsection: high-dimensional consistency proof} of the supplementary material.

\begin{theorem}\label{theorem: high-dimensional consistency of ARGES}
Assume (A1) - (A6). Let $\hat{\mathcal C}_n$, $\breve{\mathcal C}_n$ and $\tilde{\mathcal C}_n$ be the outputs of ARGES-CIG and ARGES-skeleton and GES respectively, with the scoring criterion $\mathcal{S}_{\lambda_n}$. Then there exists a sequence $\lambda_n \rightarrow 0$ such that \vspace{-0.1in}\textcolor{red}{$$\underset{n \rightarrow \infty}{\lim}~\Prob(\hat{\mathcal{C}}_n = \mathcal{C}_{n0}) = \underset{n \rightarrow \infty}{\lim}~\Prob(\breve{\mathcal{C}}_n = \mathcal{C}_{n0})  = \underset{n \rightarrow \infty}{\lim}~\Prob(\tilde{\mathcal{C}}_n = \mathcal{C}_{n0}) = 1.$$}
\end{theorem}
%\begin{theorem}\label{theorem: high-dimensional consistency of ARGES-skeleton}
%Assume (A1) - (A6). Let $\breve{\mathcal C}_n$ be the output of ARGES-skeleton with the scoring criterion $\mathcal{S}_{\lambda_n}$. Then there exists a sequence $\lambda_n \rightarrow 0$ such that \textcolor{red}{$\underset{n \rightarrow \infty}{\lim}~\Prob(\hat{\mathcal{C}}_n = \mathcal{C}_{n0}) \rightarrow 1$}.
%\end{theorem}
%
%\begin{theorem}\label{theorem: high-dimensional consistency of GES}
%Assume (A1), (A2), (A3), (A5) and (A6). Let $\tilde{\mathcal C}_n$ be the output of GES with the scoring criterion $\mathcal{S}_{\lambda_n}$. Then there exists a sequence $\lambda_n \rightarrow 0$ such that \textcolor{red}{$\underset{n \rightarrow \infty}{\lim}~\Prob(\tilde{\mathcal{C}}_n = \mathcal{C}_{n0}) \rightarrow 1$}.
%\end{theorem}
We choose $\lambda_n = \frac{1}{9}\log(1 - c_n^2)$ to prove the above theorems (see Section \ref{A2-subsection: high-dimensional consistency proof} of the supplementary material), where $c_n$ is as in (A6).
% [AH: this must be (A6), not (A5), right?]
However, similar arguments hold for any sequence $\{\lambda_n\}$ satisfying $\lambda_n < \frac{1}{8}\log(1 - c_n^2)$ and $\frac{K_nq_n\log(p_n)}{n\lambda_n}\rightarrow 0$, where $p_n$, $q_n$ and $K_n$ are as in (A2), (A3) and (A5) respectively. The penalty parameter of the BIC criterion (see Remark \ref{remark: BIC}), which is known to be weak for sparse high-dimensional settings (see, for example, \cite{FoygelDrton10}), does not satisfy $\frac{K_nq_n\log(p_n)}{n\lambda_n}\rightarrow 0$, except for some very restricted choices of $\{p_n\}$, $\{q_n\}$ and $\{K_n\}$. Further, we note that \cite{VandeGeerBuhlmann13} proved their high-dimensional consistency result with $\lambda_n = \mathcal{O}(\sqrt{\log(p_n)/n})$. This choice of $\{\lambda_n\}$ satisfies $\frac{K_nq_n\log(p_n)}{n\lambda_n}\rightarrow 0$ under (A1) - (A6), when the constant $b_2$ in (A5) is greater than $1/2$.



%\begin{remark}
%Note that our proof of Theorem \ref{theorem: high-dimensional consistency of ARGES} can easily be modified to show high-dimensional consistency of GES under similar assumptions. (A5) for GES roughly states that for large enough $\lambda$, GES ``rarely" leaves the search space defined by the estimated CIG.
%\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\subsection{Extension to the nonparanormal family of distributions}\label{subsection: nonparanormal family}

{\color{red}
\subsection{Assumption (A5)}\label{subsection: assumption A5}
% [AH: what about a more meaningful subsection title? I'd suggest something like: 'Discussion on the bound for the growth of the oracle version'.]
We first consider (A5) for $\{\delta_n\} = 0$. Then (A5) roughly states that the oracle forward phase of (AR)GES does not add ``too many" edges that do not belong to the CPDAG-skeleton. In Section \ref{A2-section: verifying (A5)}
% [AH: this isn't rendered correctly in the PDF you sent ('Section ??').
of the supplementary material, we empirically verify this in certain sparse high-dimensional settings and we find that in all but very few cases the maximum degree of the outputs of the oracle forward phase of (AR)GES are reasonably close to the maximum degree of the true CPDAG-skeleton. Further, note that (A5) is slightly different for GES, ARGES-CIG and ARGES-skeleton (see Figure \ref{A2-fig: boxplots of max degree} of the supplementary material).

The intuition for having a $\delta_n$-optimal oracle version in (A5), with $\delta_n >0$ is the following: If
$$
  |\rho(\mathcal{C}_\text{current},\mathcal{C}_\text{new}) |  \geq \underset{\mathcal{C} \in \mathfrak{C}}{\max} |\rho(\mathcal{C}_\text{current},\mathcal{C}) | - \delta_n
$$
% [AH: nitpick: I'd suggest to have this as a standalone formula, or, if kept inline, to use \max_{\mathcal{C} \in \mathfrak{C}} instead of \underset{\mathcal{C} \in \mathfrak{C}}{\max} to not break the line flow.
(see Definition \ref{definition: oracle versions of ARGES}), then the move from $\mathcal{C}_\text{current}$ to $\mathcal{C}_\text{new}$ is so close to the optimal move that it cannot be identified as sub-optimal in the sample version.

We note that the output of a $\delta_n$-optimal oracle forward phase of (AR)GES depends not only on the structure $\mathcal{C}_{n0}$ but also on the absolute values of the nonzero partial correlations (even for $\delta_n =0$). The latter makes it very difficult to characterize a family of distributions for which (A5) holds. However, we provide two strong structural conditions under which (A5) holds. The conditions are based on the following two results.

\begin{theorem}\label{theorem: disconnected nodes}
If two nodes $X_{ni}$ and $X_{nj}$ are not connected by a path in $\mathcal{C}_{n0}$, then the output of a $\delta_n$-optimal oracle forward phase of (AR)GES does not contain an edge between $X_{ni}$ and $X_{nj}$.
\end{theorem}

\begin{theorem}\label{theorem: forest}
If $\skeleton(\mathcal{C}_{n0})$ is a forest (i.e.\ contains no undirected cycle), then the output of the oracle forward phase of (AR)GES equals $\mathcal{C}_{n0}$.
\end{theorem}

% [AH: given that the proof of one of them is 'trivial' as you write, should we call them 'Lemma' instead of 'Theorem'?]

The proof of Theorem \ref{theorem: disconnected nodes} is trivial, since if $X_{ni}$ and $X_{nj}$ are not connected by a path in $\mathcal{C}_{n0}$, then $\rho_{nij|S} = 0$ for all $S \subseteq\{1,\ldots,p_n\}\setminus \{i,j\}$. Further, note that Theorem \ref{theorem: disconnected nodes} implies that it is sufficient to prove Theorem \ref{theorem: forest} when $\skeleton(\mathcal{C}_{n0})$ is an undirected tree (i.e.\ a connected graph containing no cycle) or equivalently, when $\mathcal{G}_{n0}$ is a polytree (i.e.\ a directed graph whose skeleton is an undirected tree).

%Theorem \ref{theorem: forest} implies that the oracle version of (AR)GES does not require the backward phase when $\skeleton(\mathcal{C}_{n0})$ is an undirected tree.

We note that this result shows a connection between GES and the Chow-Liu algorithm \citep{ChowLiu68} for multivariate Gaussian distributions. The Chow-Liu algorithm is a greedy forward search procedure for learning undirected trees, based on mutual information between pairs of variables (which equals $-\frac{1}{2}\log(1-\rho_{ij}^2)$ for a multivariate Gaussian distribution). Our result shows that the oracle forward phase of GES is a greedy forward search procedure for learning polytrees, based on conditional mutual information $-\frac{1}{2}\log(1-\rho_{ij|S}^2)$. To our knowledge, this connection between GES and the Chow-Liu algorithm cannot be found in the literature on the Chow-Liu algorithm and extensions thereof for learning polytrees \citep{RebanePearl87, HuetedeCampos93, deCampos98, OuerdEtAl04}.
% [AH: suggestion to reformulate; backup of previous phrasing in the comment below.]
% Although there are some extensions of the Chow-Liu algorithm for learning polytrees \citep{RebanePearl87, HuetedeCampos93, deCampos98, OuerdEtAl04}, but we were unable to find this connection between GES and the Chow-Liu algorithm in the literature.\\

We are now ready to state our sufficient conditions as the following immediate corollaries of Theorems \ref{theorem: disconnected nodes} and \ref{theorem: forest}.

\begin{corollary}\label{corollary: disconnected nodes}
If the number of nodes in each connected component of $\mathcal{C}_{n0}$ is bounded by $q_n'$ satisfying $q_n' = \mathcal{O}(n^{a'})$ for some $0 \leq a' <1$, then the maximum degree in the output of a $\delta_n$-optimal oracle forward phase of (AR)GES is bounded by $q_n'$ for all $\delta_n \geq 0$.
\end{corollary}

\begin{corollary}\label{corollary: forest}
If $\skeleton(\mathcal{C}_{n0})$ is a forest, then the maximum degree in the output of the oracle forward phase of (AR)GES equals $q_n$, where $q_n$ is given by (A3).
\end{corollary}


In order to extend Theorem \ref{theorem: forest} or Corollary \ref{corollary: forest} to a $\delta_n$-optimal version of (AR)GES, we need the following additional assumption.

\begin{description}
\item[(A7)] (bounds on the gap between simple correlations and first order partial correlations) \vspace{-0.1in}$$\underset{(i, j, k) \in T}{\inf}~  \{||\rho_{nij | k}| - |\rho_{nij}|| : |\rho_{nij | k}| \neq |\rho_{nij}|\}  \geq c_n',$$ where $T = \{(i,j,k) : \text{$(X_{ni},X_{nj},X_{nk})$ is an unshielded triple in $\mathcal{C}_{n0}$} \}$ and $c_n' \to 0$ such that $c_n^{\prime -1} = \mathcal{O}(n^{d_3})$ for some $0\leq d_3 < b_1/2$ where $b_1$ is given by (A3).
\end{description}

\begin{theorem}\label{theorem: forest 2}
Assume (A6) with $K_n = 1$ and (A7). If $\skeleton(\mathcal{C}_{n0})$ is a forest, then the output of a $\delta_n$-optimal oracle forward phase of (AR)GES equals $\mathcal{C}_{n0}$ for all $\delta_n < \min((1-M)c_n,c_n')$, where $M$ and $c_n$ are given by (A6) and $c_n'$ is given by (A7). Hence, (A5) holds with $b_2 =b_1$ and $d_1 = \max(d_2,d_3)$, where $b_1$ is given by (A3).
\end{theorem}

\begin{remark}
An obvious extension of Corollary \ref{corollary: disconnected nodes} and Theorem \ref{theorem: forest 2} is the following: if the assumption of Corollary \ref{corollary: disconnected nodes} holds for the connected components of $\skeleton(\mathcal{C}_{n0})$ that are not trees and the assumptions of Theorem \ref{theorem: forest 2} hold for the connected components of $\skeleton(\mathcal{C}_{n0})$ that are trees, then (A5) holds with $b_2=a'$ and $d_1 = \max(d_2,d_3)$.
\end{remark}

% It is an interesting result in itself, and to the best of our knowledge it was not known in the literature.

%The first condition is that the maximum size of the connected components of $\mathcal{C}_{n0}$ is $\mathcal{O}(n^{a\prime})$ for some $0 \leq a <1$

%We conclude this section by providing some sufficient conditions






%The output of an $\delta_n$-optimal oracle forward phase of (AR)GES additionally depend on the absolute difference





%Finally, note that (A5) is slightly different for GES, ARGES-CIG and ARGES-skeleton (see Figure \ref{A2-fig: boxplots of max degree} of the supplementary material).







%We note that if $p_n = \mathcal{O}(n^{a})$ for some $0 \leq a < 1$, then Assumption (A5) automatically holds with $b_2 = (1 - a)$.
}

















